Hybrid Data-Driven and Analytical Model for Kinematic Control of a Surgical Robotic Tool

Accurate kinematic models are essential for effective control of surgical robots. For tendon driven robots, which is common for minimally invasive surgery, intrinsic nonlinearities are important to consider. Traditional analytical methods allow to build the kinematic model of the system by making certain assumptions and simplifications on the nonlinearities. Machine learning techniques, instead, allow to recover a more complex model based on the acquired data. However, analytical models are more generalisable, but can be over-simplified; data-driven models, on the other hand, can cater for more complex models, but are less generalisable and the result is highly affected by the training dataset. In this paper, we present a novel approach to combining analytical and data-driven approaches to model the kinematics of nonlinear tendon-driven surgical robots. Gaussian Process Regression (GPR) is used for learning the data-driven model and the proposed method is tested on both simulated data and real experimental data.

==> KineControl.tex <==
\section{Inverse Kinematic Control}\label{sec:KineControl}
% The goal of inverse kinematics control is to have a robot follow a desired trajectory and reach a target configuration.
% % Generally, solving the inverse kinematics problem at the velociy level (thus taking the motor/joint velocities as control variables) leads to some simplification thanks to the linearization of the problem. The problem can then be formulated as
% % \begin{equation}
% % \mathbf{\dot{\theta}_t = \argmin_{\dot{\theta}_t}\frac{1}{2}||\dot{\tilde{P}}_t-\dot{P}_t||^2}
% % \end{equation}
% % where $\mathbf{\dot{\tilde{P}}_t}$ is the desired  Cartesian velocity at the time instant $t$.
% In many works researchers have been focusing on directly learning the inverse kinematics of a system. However, the knowledge of the forward kinematic model allows to guarantee better error convergence. As a matter of fact, solving
% \begin{equation} \label{eq:minProblem}
% \mathbf{\dot{\theta}_t = \argmin_{\dot{\theta}_t}\frac{1}{2}||\dot{\tilde{P}}_t-\dot{P}_t+K_p (\tilde{P}_t-P_t)||^2}
% \end{equation} 
% guarantees that the position error ($\mathbf{e =\tilde{P}_t-P_t}$) dynamics is described by $\mathbf{\dot{e} +K_p e = 0}$.

% Equation (\ref{eq:minProblem}) is however highly nonlinear in the control input, especially because of the nonlinear model from the Gaussian Process regression. Nevertheless, if small velocities are guaranteed the following can be assumed:
% \begin{equation}\label{eq:linearized}
%      \mathbf{P_t} \simeq \mathbf{P_{t-1}}+\frac{\mathbf{\partial P}}{\partial\Theta}\Big|_{t-1}d{\Theta}_t\\ ,
% \end{equation}
% where
% \begin{equation}
%     \frac{\mathbf{\partial P}}{\partial \Theta} = \begin{bmatrix}
%     \frac{\mathbf{\partial P}}{\partial \theta} &
%     \frac{\mathbf{\partial P}}{\partial \dot{\theta}} &
%     \frac{\mathbf{\partial P}}{\partial \ddot{\theta}} &
%     \frac{\mathbf{\partial P}}{\partial \theta_{old}} &
%     \frac{\mathbf{\partial P}}{\partial \dot{\theta}_{old}}
%     \end{bmatrix}
% \end{equation}
% and
% \begin{equation}
%     d\Theta_t = 
%     \begin{bmatrix} 
%     d\theta_t \\
%     d\dot{\theta}_t \\
%     d\ddot{\theta}_t \\
%     d\theta_{old,t}\\
%     d\dot{\theta}_{old,t}
%     \end{bmatrix} =
%     \begin{bmatrix}
%     \theta_t-\theta_{t-1} \\
%     \dot{\theta}_t-\dot{\theta}_{t-1}\\
%     \frac{{\dot{\theta}_t-\dot{\theta}_{t-1}}}{dt}-
%     \frac{{\dot{\theta}_{t-1}-\dot{\theta}_{t-2}}}{dt} \\
%     \theta_{t-1}-\theta_{t-2} \\
%     \dot{\theta}_{t-1}-\dot{\theta}_{t-2} \\
%     \end{bmatrix}
% \end{equation}
% Consequently, the solution of the control problem (\ref{eq:minProblem}) with the proposed linearization can be computed as
% \begin{equation}
%     \mathbf{\dot{\theta}_t = \hat{J}_t^\ssymbol{2} (I+K_p)^{-1}(\dot{\tilde{P}}_t-\frac{\hat{P}_{t-1}}{dt}+K_p(\tilde{P}_t-P_{t-1}-\hat{P}_{t-1}))}dt\ ,
% \end{equation}
% with $\ssymbol{2}$ indicating the pseudoineverse operator and 
% \begin{equation}
%     \begin{aligned}
%   & \mathbf{\hat{J}_t = \frac{\partial P}{\partial \dot{\theta}}\Big |_{t-1}
%   +\frac{\partial P}{\partial \ddot{\theta}}\Big|_{t-1}}\frac{1}{dt} \\
%   & \mathbf{\hat{P}_{t-1}} = \frac{\mathbf{\partial P}}{\partial \Theta}\Big |_{t-1}
%   \begin{bmatrix}
%   d\theta_t \\
%   -\dot{\theta}_{t-1} \\
%   \frac{\dot{\theta}_{t-2}-2\dot{\theta}_{t-1}}{dt}\\
%   d\theta_{old,t}\\
%   d\dot{\theta}_{old,t}
%   \end{bmatrix}
%     \end{aligned}
% \end{equation}


